Rawlsian Fairness in Online Bipartite Matching: Two-sided, Group, and Individual

Online bipartite-matching platforms are ubiquitous and find applications in important areas such as crowdsourcing and ridesharing. In the most general form, the platform consists of three entities: two sides to be matched and a platform operator that decides the matching. The design of algorithms for such platforms has traditionally focused on the operator's (expected) profit. Since fairness has become an important consideration that was ignored in the existing algorithms a collection of online matching algorithms have been developed that give a fair treatment guarantee for one side of the market at the expense of a drop in the operator's profit. In this paper, we generalize the existing work to offer fair treatment guarantees to both sides of the market simultaneously, at a calculated worst case drop to operator profit. We consider group and individual Rawlsian fairness criteria. Moreover, our algorithms have theoretical guarantees and have adjustable parameters that can be tuned as desired to balance the trade-off between the utilities of the three sides. We also derive hardness results that give clear upper bounds over the performance of any algorithm.

==> conclusion.tex <==
\section{Conclusion}
%\SE{update}
In this paper, we considered the problem of two-sided fairness in online matching platforms where there are three participating entities: the platform and the two sides to be matched. Unlike previous work where the fairness guarantees are provided for one particular entity, we give fairness guarantees to both offline and online sides of the matching simultaneously at a bounded drop to the platform operator's profit. We considered both group and individual fairness objectives. Our algorithms have theoretical guarantees and involve three tunable parameters which can be adjusted according to the utility trade-off desired. In addition, we showed hardness results which impose upper bounds on the achievable competitive ratios of any algorithm. 

% Finally, the results of our experiments on the NYC dataset are in accordance with our theoretical claims and show the effectiveness of our algorithm in a real-world setting. We strongly believe that this model is general enough and can be applied effectively to datasets from other applications such as crowdsourcing or online dating. 
